Five key exoplanet questions answered via the analysis of 25 hot Jupiter atmospheres in eclipse

Population studies of exoplanets are key to unlocking their statistical properties. So far the inferred properties have been mostly limited to planetary, orbital and stellar parameters extracted from, e.g., Kepler, radial velocity, and GAIA data. More recently an increasing number of exoplanet atmospheres have been observed in detail from space and the ground. Generally, however, these atmospheric studies have focused on individual planets, with the exception of a couple of works which have detected the presence of water vapor and clouds in populations of gaseous planets via transmission spectroscopy. Here, using a suite of retrieval tools, we analyse spectroscopic and photometric data of 25 hot Jupiters, obtained with the Hubble and Spitzer Space Telescopes via the eclipse technique. By applying the tools uniformly across the entire set of 25 planets, we extract robust trends in the thermal structure and chemical properties of hot Jupiters not obtained in past studies. With the recent launch of JWST and the upcoming missions Twinkle, and Ariel, population based studies of exoplanet atmospheres, such as the one presented here, will be a key approach to understanding planet characteristics, formation, and evolution in our galaxy.

==> figset_eclipse.tex <==
\figsetstart
\figsetnum{2}
\figsettitle{Fitted spectra eclipse}

\figsetgrpstart
\figsetgrpnum{2.1}
\figsetgrptitle{Image of CO1}
\figsetplot{CoRoT-1 b_spectrum_free.pdf}
\figsetgrpnote{Retrieved eclipse spectrum (left) and temperature structure (right) for the full retrievals}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.2}
\figsetgrptitle{Image of HP7}
\figsetplot{HAT-P-7 b_spectrum_free.pdf}
\figsetgrpnote{Retrieved eclipse spectrum (left) and temperature structure (right) for the full retrievals}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.3}
\figsetgrptitle{Image of HP32}
\figsetplot{HAT-P-32 b_spectrum_free.pdf}
\figsetgrpnote{Retrieved eclipse spectrum (left) and temperature structure (right) for the full retrievals}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.4}
\figsetgrptitle{Image of HP41}
\figsetplot{HAT-P-41 b_spectrum_free.pdf}
\figsetgrpnote{Retrieved eclipse spectrum (left) and temperature structure (right) for the full retrievals}
\figsetgrpend

\figsetend

\begin{figure}
\figurenum{2}
\plotone{CoRoT-1 b_spectrum_free.pdf}
\caption{Retrieved eclipse spectrum (left) and temperature structure (right) for the full retrievals}
\end{figure}

==> figset_lc.tex <==
\figsetstart
\figsetnum{1}
\figsettitle{Reduced white light-curves obtained with \emph{Iraclis} for the HST data.}

\figsetgrpstart
\figsetgrpnum{1.1}
\figsetgrptitle{White light-curve of CoRoT-1\,b}
\figsetplot{CoRoT-1_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.2}
\figsetgrptitle{White light-curve of HAT-P-2\,b}
\figsetplot{HAT-P-2_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.3}
\figsetgrptitle{White light-curve of HAT-P-7\,b}
\figsetplot{HAT-P-7_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.4}
\figsetgrptitle{White light-curve of HAT-P-32\,b}
\figsetplot{HAT-P-32_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.5}
\figsetgrptitle{White light-curve of HAT-P-41\,b}
\figsetplot{HAT-P-41_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.6}
\figsetgrptitle{White light-curve of HD\,189733\,b}
\figsetplot{HD189733_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.7}
\figsetgrptitle{White light-curve of HD\,209458\,b}
\figsetplot{HD209458_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.8}
\figsetgrptitle{White light-curve of KELT-1\,b}
\figsetplot{KELT-1_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.9}
\figsetgrptitle{White light-curve of KELT-7\,b}
\figsetplot{KELT-7_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.10}
\figsetgrptitle{White light-curve of KELT-9\,b}
\figsetplot{KELT-9_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.11}
\figsetgrptitle{White light-curve of TrES-3\,b}
\figsetplot{TRES-3_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.12}
\figsetgrptitle{White light-curve of WASP-4\,b}
\figsetplot{WASP-4_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.13}
\figsetgrptitle{White light-curve of WASP-12\,b}
\figsetplot{WASP-12_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.14}
\figsetgrptitle{White light-curve of WASP-18\,b}
\figsetplot{WASP-18_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.15}
\figsetgrptitle{White light-curve of WASP-19\,b}
\figsetplot{WASP-19_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.16}
\figsetgrptitle{White light-curve of WASP-43\,b}
\figsetplot{WASP-43_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.17}
\figsetgrptitle{White light-curve of WASP-74\,b}
\figsetplot{WASP-74_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.18}
\figsetgrptitle{White light-curve of WASP-76\,b}
\figsetplot{WASP-76_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.19}
\figsetgrptitle{White light-curve of WASP-77\,A\,b}
\figsetplot{WASP-77_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.20}
\figsetgrptitle{White light-curve of WASP-79\,b}
\figsetplot{WASP-79_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.21}
\figsetgrptitle{White light-curve of WASP-103\,b}
\figsetplot{WASP-103_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.22}
\figsetgrptitle{White light-curve of WASP-121\,b (G141)}
\figsetplot{WASP-121_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.23}
\figsetgrptitle{White light-curve of WASP-121\,b (G102)}
\figsetplot{WASP-121_G102_LC.png}
\figsetgrpnote{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}
\figsetgrpend

\figsetend

\begin{figure*}
\figurenum{1}
\plotone{CoRoT-1_LC.png}
\caption{White light-curve fit with \emph{Iraclis} (Top) and residuals (Bottom)}\label{figset:LC}
\end{figure*}


==> figset_slc.tex <==
\figsetstart
\figsetnum{2}
\figsettitle{Spectral light-curves obtained with \emph{Iraclis} for the HST data.}

\figsetgrpstart
\figsetgrpnum{2.1}
\figsetgrptitle{Spectral light-curve of CoRoT-1\,b}
\figsetplot{CoRoT-1_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.2}
\figsetgrptitle{Spectral light-curve of HAT-P-2\,b}
\figsetplot{HAT-P-2_LC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.3}
\figsetgrptitle{Spectral light-curve of HAT-P-7\,b}
\figsetplot{HAT-P-7_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.4}
\figsetgrptitle{Spectral light-curve of HAT-P-32\,b}
\figsetplot{HAT-P-32_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.5}
\figsetgrptitle{Spectral light-curve of HAT-P-41\,b}
\figsetplot{HAT-P-41_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.6}
\figsetgrptitle{Spectral light-curve of HD\,189733\,b}
\figsetplot{HD189733_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.7}
\figsetgrptitle{Spectral light-curve of HD\,209458\,b}
\figsetplot{HD209458_LC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.8}
\figsetgrptitle{Spectral light-curve of KELT-1\,b}
\figsetplot{KELT-1_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.9}
\figsetgrptitle{Spectral light-curve of KELT-7\,b}
\figsetplot{KELT-7_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.10}
\figsetgrptitle{Spectral light-curve of KELT-9\,b}
\figsetplot{KELT-9_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.11}
\figsetgrptitle{Spectral light-curve of TrES-3\,b}
\figsetplot{TRES-3_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.12}
\figsetgrptitle{Spectral light-curve of WASP-4\,b}
\figsetplot{WASP-4_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.13}
\figsetgrptitle{Spectral light-curve of WASP-12\,b}
\figsetplot{WASP-12_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.14}
\figsetgrptitle{Spectral light-curve of WASP-18\,b}
\figsetplot{WASP-18_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.15}
\figsetgrptitle{Spectral light-curve of WASP-19\,b}
\figsetplot{WASP-19_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.16}
\figsetgrptitle{Spectral light-curve of WASP-43\,b}
\figsetplot{WASP-43_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.17}
\figsetgrptitle{Spectral light-curve of WASP-74\,b}
\figsetplot{WASP-74_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.18}
\figsetgrptitle{Spectral light-curve of WASP-76\,b}
\figsetplot{WASP-76_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.19}
\figsetgrptitle{Spectral light-curve of WASP-77\,A\,b}
\figsetplot{WASP-77_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.20}
\figsetgrptitle{Spectral light-curve of WASP-79\,b}
\figsetplot{WASP-79_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.21}
\figsetgrptitle{Spectral light-curve of WASP-103\,b}
\figsetplot{WASP-103_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.22}
\figsetgrptitle{Spectral light-curve of WASP-121\,b (G141)}
\figsetplot{WASP-121_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.24}
\figsetgrptitle{Spectral light-curve of WASP-121\,b (G102)}
\figsetplot{WASP-121_G102_SLC.png}
\figsetgrpnote{Spectral light-curve obtained with \emph{Iraclis}.}
\figsetgrpend

\figsetend

\begin{figure*}
\figurenum{1}
\plotone{CoRoT-1_SLC.png}
\caption{Spectral light-curve obtained with \emph{Iraclis}.}\label{figset:SLC}
\end{figure*}
